Blackwell-Optimal Strategies in Priority Mean-Payoff Games

We examine perfect information stochastic mean-payoff games - a class of games containing as special sub-classes the usual mean-payoff games and parity games. We show that deterministic memoryless strategies that are optimal for discounted games with state-dependent discount factors close to 1 are optimal for priority mean-payoff games establishing a strong link between these two classes.

==> eptcsdata.tex <==
\providecommand{\event}{Angelo Montanari, Margherita Napoli, Mimmo Parente (Eds.)\\ Proceedings of GandALF 2010}
\providecommand{\volume}{25}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{7}
\providecommand{\eid}{5}

